LLMs in the Imaginarium: Tool Learning through Simulated Trial and Error

Tools are essential for large language models (LLMs) to acquire up-to-date information and take consequential actions in external environments. Existing work on tool-augmented LLMs primarily focuses on the broad coverage of tools and the flexibility of adding new tools. However, a critical aspect that has surprisingly been understudied is simply how accurately an LLM uses tools for which it has been trained. We find that existing LLMs, including GPT-4 and open-source LLMs specifically fine-tuned for tool use, only reach a correctness rate in the range of 30% to 60%, far from reliable use in practice. We propose a biologically inspired method for tool-augmented LLMs, simulated trial and error (STE), that orchestrates three key mechanisms for successful tool use behaviors in the biological system: trial and error, imagination, and memory. Specifically, STE leverages an LLM's 'imagination' to simulate plausible scenarios for using a tool, after which the LLM interacts with the tool to learn from its execution feedback. Both short-term and long-term memory are employed to improve the depth and breadth of the exploration, respectively. Comprehensive experiments on ToolBench show that STE substantially improves tool learning for LLMs under both in-context learning and fine-tuning settings, bringing a boost of 46.7% to Mistral-Instruct-7B and enabling it to outperform GPT-4. We also show effective continual learning of tools via a simple experience replay strategy.

==> sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[!hbt]
  \centering
    \includegraphics[width=0.95\linewidth]{fig/fig1.pdf}
  \caption{The proposed tool learning pipeline. The pipeline consists of two stages: exploration and exploitation. In the exploration stage, an LLM interacts with the tool and progressively gathers tool-use experiences through trial and error. Specifically, a) in each trial, the LLM comes up with plausible user queries related to the target tool, iteratively utilizes the tool execution feedback to fulfill the user query, and in the end self-reflects on the trial; b) a short-term memory consisting of the exploration trajectories of recent trials is augmented with the LLM, to encourage learning from recent fine-grained successes and failures and exploring the API in further depth; c) a long-term memory of coarse-grained trial and error experiences from the past exploration maintains progressive learning over a long horizon. In the exploitation stage, the exploration experiences are distilled into a set of tool-use examples to enhance LLM's tool-use abilities.}
\label{fig1}
\end{figure*}

Empowering large language models (LLMs) with the ability to utilize external tools is a promising way of resolving many of their inherent limitations towards generalist problem-solving agents, such as fixed knowledge storage, limited computational capacity and preciseness, and inability to take real actions~\citep{qin2023tool, mialon2023augmented}.
Since the seminal Toolformer~\citep{schick2023toolformer}, there has been a surge of research interest in tool-augmented LLMs, including collecting large-scale API repositories and various approaches to improve the tool-use abilities of LLMs~\citep{qin2023toolllm, tang2023toolalpaca, li2023api, huang2023metatool, paranjape2023art, patil2023gorilla, shen2023hugginggpt, lu2023chameleon, song2023restgpt, liang2023taskmatrix}. 

There are three main desiderata for tool-augmented LLMs: 
\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item \textbf{In-domain performance.} Given a set of tools, the LLM needs to be capable of appropriately deciding when and how to use the tools to help with its goals.
    \item \textbf{Flexibility.} Due to the rapidly expanding nature of tools, it would be ideal if the LLM could flexibly adapt to new tools in potentially different domains. 
    \item \textbf{Low cost.} It is always desired to reduce the costs of developing and maintaining tool-augmented LLMs as much as possible.
\end{itemize}
While the majority of existing work proposed tool-use frameworks that focus on the flexibility aspect~\citep{lu2023chameleon, song2023restgpt, shen2023hugginggpt, liang2023taskmatrix, qin2023toolllm, patil2023gorilla}, we note that \textit{in-domain performance} is still one of the greatest bottlenecks of tool-augmented LLMs that is somehow overlooked.
In fact, in-domain performance is a particularly important aspect in the context of tool use---during actual deployment, many tools have associated costs/budgets or may produce side effects (e.g., ticket booking/meeting schedulers) that could potentially be harmful to the user.
A system that is not sufficiently high-performing would require extensive user engagement (e.g., checking/correcting system outputs), which could cause even more labor than what it saves and gradually lose trust.

To illustrate the barriers hindering in-domain tool-use performance, there are two primary approaches for tool integration with LLMs: in-context learning (ICL), and fine-tuning with tool-use examples.
ICL-based approaches connect an LLM with a set of APIs via conditioning the LLM on the associated API documentation and examples, utilizing the in-context learning and instruction following abilities of LLMs~\citep{lu2023chameleon, song2023restgpt, shen2023hugginggpt, liang2023taskmatrix} or models specifically trained to use APIs based on documentations~\citep{qin2023toolllm, patil2023gorilla}.
In such approaches, successful tool use largely depends on the quality of the API documentation and examples, however, in many scenarios, the documentation/examples are not clear/thorough enough to cover the different use cases of the API, especially when the functionality of the API is complex/unusual.
For example, recent work reports that even GPT-4 faces difficulties when handling unusual tools and could often have trouble formulating problems in ways that elicit useful answers from plug-ins~\citep{bubeck2023sparks, davis2023testing}.
Fine-tuning-based approaches instead have the potential of distilling a much wider range of examples into the model, however, in the case of tool use, there are typically no/very few examples that accompany a new tool, and larger-scale human annotations are usually not an option due to the cost.
Towards addressing this, existing work~\citep{schick2023toolformer, patil2023gorilla, qin2023toolllm, tang2023toolalpaca} has explored employing LLMs to synthesize tool-use examples. Toolformer~\citep{schick2023toolformer} prompts an LLM with in-context demonstrations to synthesize plausible tool-use cases from a corpus. While the quality/quantity of the synthesized examples depends on the relation between the tool and the corpus, the approach suffers from a generally low sample efficiency as noted by the authors. \citet{patil2023gorilla, qin2023toolllm, tang2023toolalpaca} instead use an LLM to synthesize tool-use examples directly. However, their main focus is on improving the model’s ability to adapt to new APIs via documentation, and there is still considerable room for improvements in the diversity and comprehensiveness of the synthesized examples for the tools being integrated. 

In contrast to existing approaches, humans typically master tools by actively trying the tool and learning through progressive interaction and reinforcement, with potential neurocognitive basis~\citep{orban2014neural, REYNAUD2016421}. Inspired by this, we propose a new tool-learning pipeline where an LLM continually learns tools through trial and error. When a new set of APIs comes along, instead of deploying the model by conditioning on the API documentation, our pipeline goes through 1) an exploration stage where the LLM extensively interacts with the tool, with two memory mechanisms designed to dynamically grow trial-and-error experiences which enable continual and progressive tool learning with better diversity and comprehensiveness; 2) an exploitation stage where the gathered experiences are distilled into a set of tool-use examples that are utilized via either fine-tuning or as demonstration pool for ICL to enhance LLMs' tool-use ability. We conduct experiments on ToolBench\footnote{https://github.com/OpenBMB/ToolBench}, and show that our proposed framework could greatly enhance the LLM's tool-use performance, and also that fine-tuning is much more effective than ICL in equipping LLMs with tools, presumably because fine-tuning allows distilling a much larger set of experiences into the model. While vanilla fine-tuning would cause catastrophic forgetting which limits the flexibility aspect, we show that a simple experience replay strategy~\citep{scialom-etal-2022-fine} could largely mitigate the issue, allowing the model to continually learn new tools while preserving its previously acquired skills.

\begin{figure*}[t]
  \centering
    \includegraphics[width=1.0\linewidth]{fig/fig_mem.pdf}
  \caption{Exploration with simulated trial and error, highlighting the memory mechanisms. Each episode begins with the API specification (only in the first trial), followed by a series of trials dynamically added in the short-term memory. The long-term memory is loaded into the context at the beginning of every trial to allow the LLM to progressively imagine novel scenarios, and then offloaded afterward (omitted in the figure).}\Jason{A few suggestions to improve the figure, which has great content but is a bit confusing when I try to understand the prompt format.  (1) I think the API name and description only appear at the start of each episode and are not repeated at the start of each trial.  So shouldn't they appear before the label "Trial 1"?   Or perhaps they appear at the start of Trial 1 only, and the instruction "Now based on what you have discovered ..." appears at the start of all trials $> 1$?  This isn't clear from the figure itself; so you can explain in the caption if necessary.
  (2) Isn't this also true of Long-Term Memory---it is not repeated at the start of each trial? (The main text says that it is, but surely that would be a waste of prompt space \ldots ?) (3) The bottom part of the right panel is short-term memory again, right?  So can you label it as such?  This makes it clear that the right side is not showing LTM, as the reader might otherwise think, but is showing Episode N with both LTM and STM.  I suggest using a bracket in the left panel to delineate the "Query" through "Self-reflection" portion as a short-term memory.  You can then use the same kind of bracket in the right panel.  The caption should clarify that LTM is omitted in episode 1 but appears at the start of all subsequent episodes---is that right?}
\label{fig:mem}
\end{figure*}

